The frequency of extreme X-ray variability of radio-quiet quasars

We analyze 1598 serendipitous Chandra X-ray observations of 462 radio-quiet quasars to constrain the frequency of extreme amplitude X-ray variability that is intrinsic to the quasar corona and innermost accretion flow. The quasars in this investigation are all spectroscopically confirmed, optically bright ($m_i \leq$ 20.2), and contain no identifiable broad absorption lines in their optical/ultraviolet spectra. This sample includes quasars spanning $z \approx$ 0.1 - 4 and probes X-ray variability on timescales of up to $\approx$ 12 rest-frame years. Variability amplitudes are computed between every epoch of observation for each quasar and are analyzed as a function of timescale and luminosity. The tail-heavy distributions of variability amplitudes at all timescales indicate that extreme X-ray variations are driven by an additional physical mechanism and not just typical random fluctuations of the coronal emission. Similarly, extreme X-ray variations of low-luminosity quasars seem to be driven by an additional physical mechanism, whereas high-luminosity quasars seem more consistent with random fluctuations. The amplitude at which an X-ray variability event can be considered extreme is quantified for different timescales and luminosities. Extreme X-ray variations occur more frequently at long timescales ( $\Delta t \gtrsim$ 300 days) than at shorter timescales, and in low-luminosity quasars compared to high-luminosity quasars over a similar timescale. A binomial analysis indicates that extreme intrinsic X-ray variations are rare, with a maximum occurrence rate of <2.4% of observations. Finally, we present X-ray variability and basic optical emission-line properties of three archival quasars that have been newly discovered to exhibit extreme X-ray variability.

==> schema.tex <==
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
  \multicolumn{1}{|c|}{NAME} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{$z$} &
  \multicolumn{1}{c|}{ObsID} &
  \multicolumn{1}{c|}{Net Full\_cts} &
  \multicolumn{1}{c|}{TSTART} \\
\hline
  02h10m00.2188s-10d03m54.2869s & 32.5009 & -10.0650 & 1.976 & 15666 & 238.225 & 4.905E8\\
  02h10m00.2188s-10d03m54.2869s & 32.5009 & -10.0650 & 1.976 & 15667 & 486.303 & 4.907E8\\
  09h57m32.0435s+02d43m01.782s & 149.3835 & 2.7171 & 0.849 & 15258 & 284.474 & 5.050E8\\
  09h57m32.0435s+02d43m01.782s & 149.3835 & 2.7171 & 0.849 & 15259 & 274.178 & 5.072E8\\
  23h37m22.0166s+00d22m38.8852s & 354.3417 & 0.3774 & 1.382 & 3248 & 9.930 & 1.425E8\\
  23h37m22.0166s+00d22m38.8852s & 354.3417 & 0.3774 & 1.382 & 11728 & 27.384 & 3.669E8\\
\hline\end{tabular}

